Compression-aware Training of Deep Networks

In recent years, great progress has been made in a variety of application domains thanks to the development of increasingly deeper neural networks. Unfortunately, the huge number of units of these networks makes them expensive both computationally and memory-wise. To overcome this, exploiting the fact that deep networks are over-parametrized, several compression strategies have been proposed. These methods, however, typically start from a network that has been trained in a standard manner, without considering such a future compression. In this paper, we propose to explicitly account for compression in the training process. To this end, we introduce a regularizer that encourages the parameter matrix of each layer to have low rank during training. We show that accounting for compression during training allows us to learn much more compact, yet at least as effective, models than state-of-the-art compression techniques.

==> rebuttal.tex <==
\section{Rebuttal}
We thank the reviewers for their positive comments regarding the interest, novelty and quality of the paper. 

{\bf To All: Experiments.} We originally thought there was a separate deadline for supplementary material, which explains why some experiments are missing. Below, we provide the results of the experiments suggested by the reviewers. We will include these experiments in our paper.

Comparison with [14] (R1 and R2): On ICDAR, the baseline (using SGD and L2 regularization) has 3.7M parameters and a top-1 accuracy of 88.6\%. The post-processing of [14] with $e_l$ = 90\% yields a similar accuracy with 3.6M parameters. Our model, with $\tau = 15$ and no group-sparsity, yields an accuracy increase of 1\% for a model that has only 525K parameters. Interestingly, we also found that pruning the model after 25 epochs (instead of 55 originally) and reloading and training the pruned model lead to an improved accuracy of 90.46\% with again 525K parameters.

Comparison with [2] (R1, R2 and R3): On the same ICDAR experiment as above, [2] obtains a top-1 accuracy of 88.8\% with 728K parameters. Combining our low-rank regularizer with group-sparsity, we obtain an accuracy of 89.73\% with only 318K parameters (and 90.52\% accuracy with 454K parameters for $e_l$ = 100\%). Note that, while different results for [2] can be obtained by varying its hyper-parameter, we found the conclusions above (slightly higher accuracy with significantly fewer parameters) to hold in general.


Comparison to L1 and L2 regularizers (R2): While these regularizers may indeed zero out some weights, they act on individual parameters instead of entire units in our case. Nevertheless, we compare our approach with these baselines on the ICDAR dataset as before. Pruning the weights of the baseline models with a threshold of 0.0001 resulted in 1.5M zeroed-out parameters for the L2 regularizer and 2.8M zeroed-out parameters for the L1 regularizer sparsely located within units (neurons). Applying post-processing (low-rank approximation with $e_l=100\%$) to these experiments yielded models with 3.6M and 3.2M parameters respectively for L2 and L1 regularizers. Top-1 accuracy for these two experiments was 87\% and 89\% respectively after post-processing. Stronger L1 regularizer resulted in lower top-1 accuracy. By comparison, our approach yields a model with 3.4M zeroed-out parameters after post-processing and a top-1 accuracy of 90\%. As in the comparison with [2], the benefits of our approach hold for varying regularizer weights.


Results on large models (R3): In Fig. 3, we provided results on ImageNet with a ResNet-50 model. For post-processing we used $e_l=90\%$ for all these experiments which resulted in a similar performance. The baseline corresponds to a top-1 accuracy of 74.7\% and 18M parameters. Post-processing this baseline resulted in a compression rate of 4\%. Results using our approach (low-rank) correspond to a top-1 accuracy of 75.0\% for a compression rate of 20.6\%. When using both regularizers, group sparsity and low-rank jointly, we obtain a top-1 accuracy of 75.2\% for a compression rate of 27\%. By comparison, applying [2] to the same model yields an accuracy of 74.5\% for a compression rate of 17\%. 

{\bf To R2:}

We will include a discussion of variational inference methods in the paper. The priors and posteriors used in these approaches will typically zero out individual weights (with special cases corresponding to the L1 and L2 regularizers discussed above). It is however unclear to us how our regularizer(s) could be encoded in such a framework. Nevertheless, similarly to the paper suggested by R2, we also found that pruning the network early during training (after 25 epochs) and retraining the pruned model could further improve the performance of our method.

We agree with R2 that a graph showing accuracy vs compression ratio would be easier to understand and will therefore present our results in this manner, including the comparison to the baselines provided above.

{\bf To R3:}

Novelty: Our goal is to demonstrate the importance of accounting for compression during training. To the best of our knowledge, and as acknowledged by the other reviewers, we are the first to do this with a low-rank regularizer, which, as shown empirically, has a large impact on inference time and memory footprint. Furthermore, we found that this could also be beneficial for training, by pruning the network after only a few epochs (e.g., 15) and reloading and training the pruned network, which becomes much more efficient. Specifically, on ICDAR, using a combination of low-rank and group-sparsity, we were able to reduce the training time (with batch size of 32 and training for 100 epochs) from 1.69 to 0.77 hours (relative speedup of 54.5\%). The accuracy also improved by 2\% and the number of parameters reduced from 3.7M (baseline) to 208K (relative 94\% reduction). We found this behavior to be stable across a wide range of regularization parameters. By varying the epoch at which reloading occurred (from 55 to 15), we obtained compression rates ranging from 84\% to 94\% (590K to 208K parameters) for minor accuracy variations. If we seek to maintain accuracy compared to the baseline, we found that we could achieve a compression rate of 95.5\% (up to 96\% for an accuracy drop of 0.5\%), which corresponds to a training time reduced by up to 60\%.

Comparison to [18]:The pruning step of [18] performs a post-processing to remove the parameters with small weights, which essentially correspond to the baselines with L1 and L2 regularizers discussed above, and is thus not as effective as our approach. The other steps (quantization and Huffman coding) could also be applied to our approach.

